Iterable Forward Reachability Analysis of Monitor-DPNs

There is a close connection between data-flow analysis and model checking as observed and studied in the nineties by Steffen and Schmidt. This indicates that automata-based analysis techniques developed in the realm of infinite-state model checking can be applied as data-flow analyzers that interpret complex control structures, which motivates the development of such analysis techniques for ever more complex models. One approach proposed by Esparza and Knoop is based on computation of predecessor or successor sets for sets of automata configurations. Our goal is to adapt and exploit this approach for analysis of multi-threaded Java programs. Specifically, we consider the model of Monitor-DPNs for concurrent programs. Monitor-DPNs precisely model unbounded recursion, dynamic thread creation, and synchronization via well-nested locks with finite abstractions of procedure- and thread-local state. Previous work on this model showed how to compute regular predecessor sets of regular configurations and tree-regular successor sets of a fixed initial configuration. By combining and extending different previously developed techniques we show how to compute tree-regular successor sets of tree-regular sets. Thereby we obtain an iterable, lock-sensitive forward reachability analysis. We implemented the analysis for Java programs and applied it to information flow control and data race detection.

==> eptcsdata.tex <==
\providecommand{\firstpage}{384}
\providecommand{\publicationstatus}{A. Banerjee, O. Danvy, K.-G. Doh, J. Hatcliff (Eds):\\
David A. Schmidt's 60th Birthday Festschrift\\
EPTCS 129, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.129.24}{10.4204/EPTCS.129.24}}
\pdfoutput=1

